Fast Private Location-based Information Retrieval Over the Torus

Location-based services offer immense utility, but also pose significant privacy risks. In response, we propose LocPIR, a novel framework using homomorphic encryption (HE), specifically the TFHE scheme, to preserve user location privacy when retrieving data from public clouds. Our system employs TFHE's expertise in non-polynomial evaluations, crucial for comparison operations. LocPIR showcases minimal client-server interaction, reduced memory overhead, and efficient throughput. Performance tests confirm its computational speed, making it a viable solution for practical scenarios, demonstrated via application to a COVID-19 alert model. Thus, LocPIR effectively addresses privacy concerns in location-based services, enabling secure data sharing from the public cloud.

==> Section/temp.tex <==

% \caption{Overall description of ToMAS.}\label{euclid}
% % \begin{flushleft}
% % \hspace*{\algorithmicindent} \textbf{Input:} $\textbf{X,Y} \in \{0,1\}^k$, $ID, PW$, $\lambda$, $\tau$           \\
% % \hspace*{\algorithmicindent} \textbf{Output:} $d \in $ $\mathsf{\{accept,reject\}}$ \\
% % \hspace*{\algorithmicindent} \textbf{Enrollment:} An end-user $U$ registers biometric template $\textbf{X}$\\ 
% % and identity $ID$ to the authentication server $\mathcal{AS}$.
% % \end{flushleft}
% \begin{flushleft}
%     % \tcc{Cluster Assignment}
% \textbf{Input:} $\textbf{X,Y} \in \{0,1\}^k$, $ID, PW$, $\lambda$, $\tau$ \\
% \textbf{Output:} $\mathsf{accept,reject}$ \\
% \textbf{Enrollment:} An end-user $U$ registers biometric template $\textbf{X}$ and identity $ID$ to the authentication server $\mathcal{AS}$.\\
% \end{flushleft}
% \begin{algorithmic}[1]
% % \Procedure{MyProcedure}{}
% %    \Procedure{MyProcedure}{$x,y$}
% %     % Input:
% %     \Comment{Input: x}
% %     % Output:
% %     \Comment{Output:y}
% \State $U$ select parameter sets for $\lambda$ bits of security.
% \State $U$ generates pair of keys $\mathsf{(pk, sk)}\leftarrow \mathsf{KeyGen}(\lambda)$ using his/her password $PW$.
% \State $U$ encrypts biometric template $\textbf{X}$ with $\mathsf{sk}$, and sends  ($\mathsf{Enc}_{\mathsf{sk}}(\textbf{X})$, $ID$, $\mathsf{pk}$) to the $\mathcal{AS}$.
% \State The database $\mathcal{DB}$ in the $\mathcal{AS}$ stores ($\mathsf{Enc}_{\mathsf{sk}}(\textbf{X})$, $ID$, $\mathsf{pk}$). 
% \end{algorithmic}
% \begin{flushleft}
% \textbf{Authentication:} An end-user $U$ registers fresh biometric template $\textbf{Y}$ and identity $ID$ to the authentication server $\mathcal{AS}$ for an authentication.\\
% \end{flushleft}
% \begin{algorithmic}[1]
% \State $U$ select parameter sets for $\lambda$ bits of security.
% \State $U$ generates pair of keys $\mathsf{(pk, sk)}\leftarrow \mathsf{KeyGen}(\lambda)$ using his/her password $PW$.
% \State $U$ encrypts biometric template $\textbf{Y}$ with $\mathsf{sk}$, and sends  ($\mathsf{Enc}_{\mathsf{sk}}(\textbf{Y})$, $ID$) to the $\mathcal{AS}$.
% \State The database $\mathcal{DB}$ in the $\mathcal{AS}$ stores ($\mathsf{Enc}_{\mathsf{sk}}(\textbf{Y})$, $ID$).
% \State The $\mathcal{DB}$ retrives $(\mathsf{Enc}_{\mathsf{sk}}(\textbf{X}))$ and the $\mathcal{AS}$ computes hamming distance $\bar{d} \leftarrow HammingDistance(\mathsf{Enc}_{\mathsf{sk}}(\textbf{X}),\mathsf{Enc}_{\mathsf{sk}}(\textbf{Y}), \mathsf{pk})$.
% \State The $\mathcal{AS}$ sends $\bar{d}$ to the $U$ in order to partially decrypts the result $\bar{d}^{'} \leftarrow \mathsf{Par.Dec}(\bar{d},\mathsf{sk})$.
% \State The $\mathcal{AS}$ receives $\bar{d}^{'}$ from the $U$ and finally decrypts the results $d \leftarrow \mathsf{Fin.Dec}(\bar{d}^{'})$ by rounding it.
% \State The$\mathcal{AS}$ compares the result with the threshold value $\tau$ and outputs an authentication request, accept if $d < \tau$ and $reject$ otherwise $d \geq \tau$.
% \end{algorithmic}
% % \EndProcedure
% \end{algorithm}
% %

% %% overall procedure
% \begin{algorithm}[!htb]
%   \DontPrintSemicolon

%   \tcc{Preprocessing}
%   \nonl \underline{\textsc{Client}($\mathfrak{K}$)}
  
%   Sends $N$ fresh \textsf{TLWE} samples $\mathsf{ct}_i$ and \textsf{PK} to cloud

%   \nonl \underline{\textsc{Cloud}(\textsf{PK}, $\mathsf{ct}_i$)}

%   Creates service $S_i$ based on the location coordinate

%   Add $N$ number of $\mathsf{ct}_i$ to each service $S_i$

%   \tcc{Evaluation}
  
%   \nonl \underline{\textsc{Client}($\mathfrak{K}, (x, y)$)}
  
%   Receives gps data from the satellite
  
%   Encrypt $(x, y)$ with $\mathfrak{K}$

%   Sends $(\mathsf{Enc}_{\mathfrak{K}}(x), \mathsf{Enc}_{\mathfrak{K}}(y))$ to the public cloud

%   \nonl \underline{\textsc{Server}($\mathfrak{K}, (x, y)$}

  

  
  
  
% \caption{Overall Process of Our Model}
% \label{alg:overall_our_model}
% \end{algorithm}

% \begin{figure}[htb]
%     \centering
%     \begin{subfigure}[t]{0.48\textwidth}
%         % \centering
%         \includegraphics[width=\textwidth]{Figure/easy_locpir.eps}
%         \caption{(a))}
%     \end{subfigure}

%     \begin{subfigure}[t]{0.483\textwidth}
%         % \centering
%         \includegraphics[width=\textwidth]{Figure/num_locpir.eps}
%         \caption{(b))}
%     \end{subfigure}
%     \hfill

%     \caption{Easy illustration}
%     \label{fig:easy_loc}
% \end{figure}

% \begin{table*}[htb!]
% \centering
% \label{tab:performance}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Parameter Set} & \multirow{2}{*}{\textsf{Encrypt}} & \multicolumn{4}{c|}{\textsf{LocPIR}} & \multirow{2}{*}{\textsf{Decrypt}} \\
% \cline{3-6}
% & & Comparison & Valid & WBadd & Total & \\
% \hline \hline
% $\lambda_{80}$ & 1 & 2 & 2 & 1 & 1 & 1 \\
% $\lambda_{128}$ & 21 & 2 & 1 & 1 & 2 & 1 \\
% \hline
% \end{tabular}
% \caption{Performance Evaluation: with $l=13$ of precision: $2^-4$}
% \end{table*}

% \begin{table}[htb!]
% \centering
% \begin{tabular}{cccccccc}
% \toprule
% \multicolumn{1}{c}{} & \multicolumn{4}{c}{Length of Input GPS Data $(l)$} \\
% \cmidrule(lr){2-5}
% \multirow{-2}{*}{$N$} & \textbf{8-bit} & \textbf{16-bit} & \textbf{24-bit} & \textbf{32-bit} \\
% \midrule
% $1$ & $1.479$ & $2.770$ & $4.178$ & $5.453$ \\
% $2$ & $1.515$ & $2.942$ & $4.291$ & $5.648$ \\
% $3$ & $1.662$ & $3.084$ & $4.532$ & $5.920$ \\
% $4$ & $1.748$ & $3.159$ & $4.626$ & $6.071$ \\
% $5$ & $1.749$ & $3.251$ & $4.865$ & $6.445$ \\
% $6$ & $1.773$ & $3.416$ & $5.183$ & $6.369$ \\
% $7$ & $2.379$ & $4.292$ & $6.235$ & $8.169$ \\
% $8$ & $2.618$ & $4.846$ & $7.552$ & $9.392$ \\
% \bottomrule
% \end{tabular}
% \caption{performance number and length}
% \label{tab:performance_number_and_length}
% \end{table}

% \begin{table}[htb!]
% \centering
% \begin{tabular}{cccccc}
% \toprule
% $m$ & $N=4$ & $N=8$ & $N=12$ & $N=16$ \\
% \midrule
% $1$ & $0.025$ & $0.038$ & $0.050$ & $0.084$ \\
% $2$ & $0.105$ & $0.061$ & $0.191$ & $0.201$ \\
% $3$ & $0.067$ & $0.100$ & $0.165$ & $0.180$ \\
% $4$ & $0.086$ & $0.128$ & $0.180$ & $0.218$ \\
% $5$ & $0.283$ & $0.203$ & $0.208$ & $0.283$ \\
% $6$ & $0.137$ & $0.188$ & $0.268$ & $0.321$ \\
% $7$ & $0.335$ & $0.245$ & $0.363$ & $0.390$ \\
% $8$ & $0.191$ & $0.235$ & $0.342$ & $0.576$ \\
% $9$ & $0.211$ & $0.275$ & $0.372$ & $0.571$ \\
% $10$ & $0.214$ & $0.298$ & $0.444$ & $0.580$ \\
% \bottomrule
% \end{tabular}
% \caption{Table Caption}
% \label{tab:service_length}
% \end{table}
